Modeling and simulation of sector-coupled networks: A gas-power benchmark

In this contribution, we aim at presenting a gas-to-power benchmark problem that can be used for the simulation of electricity and gas networks in a time-dependent environment. Based on realistic data from the IEEE database and the GasLib suite, we describe the full set up of the underlying equations and motivate the choice of parameters. The simulation results demonstrate the applicability of the proposed approach and also allow for a clear visualization of gas-power conversion.

==> tables/flow_g2p.tex <==
\small
  \pgfplotstabletypeset[
every head row/.style={before row={\toprule},after row=\midrule,},
every last row/.style={after row=\bottomrule},
every even row/.style={before row={\rowcolor[gray]{0.85}}},
outfile=tables/flow_g2p.out.tex,
multicolumn names,
string type,
header=has colnames,
display columns/0/.style={column type={S[round-mode=places,round-precision=1]}},
display columns/1/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/2/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/3/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/4/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/5/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/6/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/7/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/8/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/9/.style={column type={S[round-mode=places,round-precision=2]}},
display columns/10/.style={column type={S[round-mode=places,round-precision=2]}},
  ]\tableflow
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:







==> tables/pressure_and_flow_g2p.tex <==



\pgfplotstableread{./figures/figuredata/gtp-ld10-N7071.table}{\tablea}
\pgfplotstableread{./figures/figuredata/gtp-ld12-N7024.table}{\tableb}
\pgfplotstableread{./figures/figuredata/gtp-ld13-N230.table }{\tablec}
\pgfplotstableread{./figures/figuredata/gtp-ld24-N221.table }{\tabled}
\pgfplotstableread{./figures/figuredata/gtp-ld29-N7061.table}{\tablee}
 \pgfplotstableread{./figures/figuredata/gtp-ld2-N7017.table }{\tablef}
\pgfplotstableread{./figures/figuredata/gtp-ld31-N213.table }{\tableg}
\pgfplotstableread{./figures/figuredata/gtp-ld36-N7001.table}{\tableh}
\pgfplotstableread{./figures/figuredata/gtp-ld42-N7039.table}{\tablei}
 \pgfplotstableread{./figures/figuredata/gtp-ld6-N7057.table }{\tablej}


\pgfplotstableset{
     create on use/t/.style={create col/copy column from table={\tablea}{t}},  
     create on use/N7071/.style={create col/copy column from table={\tablea}{p}},
     create on use/N7024/.style={create col/copy column from table={\tableb}{p}},
     create on use/N230/.style={create col/copy column from table={\tablec}{p}},
     create on use/N221/.style={create col/copy column from table={\tabled}{p}},
     create on use/N7061/.style={create col/copy column from table={\tablee}{p}},
     create on use/N7017/.style={create col/copy column from table={\tablef}{p}},
     create on use/N213/.style={create col/copy column from table={\tableg}{p}},
     create on use/N7001/.style={create col/copy column from table={\tableh}{p}},
     create on use/N7039/.style={create col/copy column from table={\tablei}{p}},
     create on use/N7057/.style={create col/copy column from table={\tablej}{p}},
}


\pgfplotstablenew[columns={t,N7071,N7024,N230,N221,N7061,N7017,N213,N7001,N7039,N7057}]{\pgfplotstablegetrowsof{\tablea}}\tablepressure
\begin{table}[ht]
  \centering
  \caption{pressure values at the gas-power conversion plants (time in hours,
    pressure in \si{\bar})}
  \small
  \pgfplotstabletypeset[
every head row/.style={before row={\toprule},after row=\midrule,},
every last row/.style={after row=\bottomrule}
  ]\tablepressure
    \label{tab:pressure-gtp}
  \end{table}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:







==> tables/pressure_g2p.tex <==
\small
\pgfplotstabletypeset[
every head row/.style={before row={\toprule},after row=\midrule,},
every last row/.style={after row=\bottomrule},
every even row/.style={before row={\rowcolor[gray]{0.85}}},
outfile=tables/pressure_g2p.out.tex,
multicolumn names,
string type,
header=has colnames,
display columns/0/.style={column type={S[round-mode=places,round-precision=1]}},
display columns/1/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/2/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/3/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/4/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/5/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/6/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/7/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/8/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/9/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
display columns/10/.style={column type={S[table-format=3.2,round-mode=places,round-precision=2]}},
]\tablepressure
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/tablesetup.tex <==
\pgfplotstableread{./figures/figuredata/gtp-ld10-N7071.table}{\tablea}
\pgfplotstableread{./figures/figuredata/gtp-ld12-N7024.table}{\tableb}
\pgfplotstableread{./figures/figuredata/gtp-ld13-N230.table}{\tablec}
\pgfplotstableread{./figures/figuredata/gtp-ld24-N221.table}{\tabled}
\pgfplotstableread{./figures/figuredata/gtp-ld29-N7061.table}{\tablee}
\pgfplotstableread{./figures/figuredata/gtp-ld2-N7017.table}{\tablef}
\pgfplotstableread{./figures/figuredata/gtp-ld31-N213.table}{\tableg}
\pgfplotstableread{./figures/figuredata/gtp-ld36-N7001.table}{\tableh}
\pgfplotstableread{./figures/figuredata/gtp-ld42-N7039.table}{\tablei}
\pgfplotstableread{./figures/figuredata/gtp-ld6-N7057.table}{\tablej}
\pgfplotstableset{
  create on use/t/.style={create col/copy column from table={\tablea}{t}},
  create on use/N7071/.style={create col/copy column from table={\tablea}{p}},
  create on use/N7024/.style={create col/copy column from table={\tableb}{p}},
  create on use/N230/.style={create col/copy column from table={\tablec}{p}},
  create on use/N221/.style={create col/copy column from table={\tabled}{p}},
  create on use/N7061/.style={create col/copy column from table={\tablee}{p}},
  create on use/N7017/.style={create col/copy column from table={\tablef}{p}},
  create on use/N213/.style={create col/copy column from table={\tableg}{p}},
  create on use/N7001/.style={create col/copy column from table={\tableh}{p}},
  create on use/N7039/.style={create col/copy column from table={\tablei}{p}},
  create on use/N7057/.style={create col/copy column from table={\tablej}{p}}
}
\pgfplotstablenew[columns={t,N7071,N7024,N230,N221,N7061,N7017,N213,N7001,N7039,N7057}]{\pgfplotstablegetrowsof{\tablea}}\tablepressure

\pgfplotstableset{
     create on use/t/.style={create col/copy column from table={\tablea}{t}},  
     create on use/N7071/.style={create col/copy column from table={\tablea}{q}},
     create on use/N7024/.style={create col/copy column from table={\tableb}{q}},
     create on use/N230/.style={create col/copy column from table={\tablec}{q}},
     create on use/N221/.style={create col/copy column from table={\tabled}{q}},
     create on use/N7061/.style={create col/copy column from table={\tablee}{q}},
     create on use/N7017/.style={create col/copy column from table={\tablef}{q}},
     create on use/N213/.style={create col/copy column from table={\tableg}{q}},
     create on use/N7001/.style={create col/copy column from table={\tableh}{q}},
     create on use/N7039/.style={create col/copy column from table={\tablei}{q}},
     create on use/N7057/.style={create col/copy column from table={\tablej}{q}}
}
\pgfplotstablenew[columns={t,N7071,N7024,N230,N221,N7061,N7017,N213,N7001,N7039,N7057}]{\pgfplotstablegetrowsof{\tablea}}\tableflow






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

